FluxEDA: A Unified Execution Infrastructure for Stateful Agentic EDA

Large language models and autonomous agents are increasingly explored for EDA automation, but many existing integrations still rely on script-level or request-level interactions, which makes it difficult to preserve tool state and support iterative optimization in real production-oriented environments. In this work, we present FluxEDA, a unified and stateful infrastructure substrate for agentic EDA. FluxEDA introduces a managed gateway-based execution interface with structured request and response handling. It also maintains persistent backend instances. Together, these features allow upper-layer agents and programmable clients to interact with heterogeneous EDA tools through preserved runtime state, rather than through isolated shell invocations. We evaluate the framework using two representative commercial backend case studies: automated post-route timing ECO and standard-cell sub-library optimization. The results show that FluxEDA can support multi-step analysis and optimization over real tool contexts, including state reuse, rollback, and coordinated iterative execution. These findings suggest that a stateful and governed infrastructure layer is a practical foundation for agent-assisted EDA automation.

==> doc/flow.tex <==
\section{Methodology}
\label{sec:flow}
In this section, we first present a physics-aware, differentiable VSB-EBL simulator. Based on this simulator, we propose a shot-level MDP optimization strategy. Finally, by integrating the MDP method with a differentiable OL simulator, we construct a unified MDP-based ILT framework.

\subsection{Physics-aware Differentiable VSB-EBL Simulation}
In VSB lithography, exposure operates shot-by-shot. The total energy deposited on the resist is obtained by summing all $N$ shots, as shown in \Cref{eq:total_energy}. The energy deposition \(E_k(x, y)\) from the \(k\)-th rectangular shot is modeled as a weighted combination of forward $(f)$ scattering and backward $(b)$ scattering components, as expressed in \Cref{eq:energy_deposition}.
\begin{equation}
E(x, y) = \sum_{k=1}^{N} E_k(x, y),
\label{eq:total_energy}
\end{equation}
\begin{equation}
E_k(x, y) = w_f E_{k, f}(x, y) + w_b E_{k, b}(x, y),
\label{eq:energy_deposition}
\end{equation}
where the weights are defined as:
\begin{equation}
w_f = \frac{1}{1+\eta}, \quad
w_b = \frac{\eta}{1+\eta}.
\label{eq:weight}
\end{equation}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{DAC26-OMPC-sub/figs/erf_new.pdf}
    \caption{(a) The erf exhibits a sigmoid-like profile. (b) 3D surface of normalized energy deposition for a single VSB shot.}
    \label{fig:erf_new}
\end{figure}

The backward scattering component $E_{k,b}(x, y)$ is modeled as the convolution of the \(k\)-th rectangular shot with a separable Gaussian PSF along the \(x\)-axis and \(y\)-axis. Due to the separability of the Gaussian PSF, this two-dimensional convolution can be expressed as the product of two one-dimensional convolutions. Each one-dimensional contribution is expressed in terms of the erf. The definition and  derivative of the erf are given by \Cref{eq:erf}. This formulation, which expresses the Gaussian PSF convolution in terms of the erf, provides a rigorous, physics-aware description of shot-level energy deposition, capturing the underlying electron-scattering process without the need for numerical approximation. The $k$-th VSB shot is represented by $(x_k, y_k, w_k, h_k, d_k, q_k)$, and its corresponding one-dimensional contributions are provided in \Cref{eq:fxfy}. The backward scattering component $E_{k,b}(x, y)$ is then obtained by combining these orthogonal terms and weighting them with the dose factor \(d_k\) and the active flag \(q_k\), as shown in \Cref{eq:Ek_sigma}. The forward scattering component $E_{k,f}(x, y)$ can be computed using a similar methodology.
\begin{equation}
\mathrm{erf}(x) = \frac{2}{\sqrt{\pi}} \int_{0}^{x} e^{-t^2} \, dt, \frac{d}{dx}\mathrm{erf}(x) = \frac{2}{\sqrt{\pi}} e^{-x^2},
\label{eq:erf}
\end{equation}

\begin{equation}
\begin{aligned}
F_{x,k}^{b} &= \tfrac{1}{2} \left[ \operatorname{erf}\!\left( \tfrac{x - x_k}{\sigma_b} \right)
     - \operatorname{erf}\!\left( \tfrac{x - (x_k + w_k)}{\sigma_b} \right) \right], \\
F_{y,k}^{b} &= \tfrac{1}{2} \left[ \operatorname{erf}\!\left( \tfrac{y - y_k}{\sigma_b} \right)
     - \operatorname{erf}\!\left( \tfrac{y - (y_k + h_k)}{\sigma_b} \right) \right],
\end{aligned}
\label{eq:fxfy}
\end{equation}
\begin{equation}
E_{k,b}(x,y) = d_k\, q_k\, F_{x,k}^{b}\, F_{y,k}^{b}.
\label{eq:Ek_sigma}
\end{equation}

As illustrated in \Cref{fig:erf_new}(a), the erf exhibits a sigmoid-like profile and is inherently differentiable, enabling exact gradient computation without artificial smoothing. \Cref{fig:erf_new}(b) shows a 3D surface plot of the normalized energy deposition for a single shot, computed by the differentiable VSB-EBL model. 


The geometric parameters of VSB shots are defined on a discrete pixel grid and therefore require integer values. The active flag $q_k$ is also binary. We employ the straight-through estimator (STE) to enforce these constraints while enabling gradient-based optimization.

Owing to the differentiability of the erf, the mapping from shot-level parameters to the pixel-level mask is fully differentiable. We define the function $g_{\sigma_f}(x, a)$ and $\Delta g_{\sigma_f}(x; x_k, w_k)$ as:
\begin{equation}
g_{\sigma_f}(x, a) = \frac{1}{\sqrt{\pi}\, {\sigma_f}} \exp\Big(-\frac{(x-a)^2}{{\sigma_f}^2}\Big),
\label{eq:g_sigma}
\end{equation}
\begin{equation}
\Delta g_{\sigma_f}(x; x_k, w_k) = g_{\sigma_f}(x, x_k + w_k) - g_{\sigma_f}(x, x_k).
\label{eq:delta_g}
\end{equation}
The corresponding $y$-direction terms, $g_{\sigma_f}(y, a)$ and $\Delta g_{\sigma_f}(y; y_k, h_k)$, as well as $g_{\sigma_b}(x, a)$, $\Delta g_{\sigma_b}(x; x_k, w_k)$, and their $y$-direction counterparts, can be defined analogously. According to the chain rule, the gradient of the energy deposition $E_(x, y)$ with respect to $x_k$ is then given by \Cref{eq:grad_xk}.
\begin{equation}
\frac{\partial E(x,y)}{\partial x_k} = d_k q_k(w_f F_{y,k}^{f} \Delta g_{\sigma_f}(x; x_k, w_k) + w_b F_{y,k}^{b} \Delta g_{\sigma_b}(x; x_k, w_k)).
\label{eq:grad_xk}
\end{equation}
The gradients with respect to $w_k$ and $d_k$ are computed using \Cref{eq:grad_wk} and \Cref{eq:grad_dk}, respectively, whereas those with respect to $y_k$, $h_k$, and $q_k$ can be derived in a similar manner.
\begin{equation}
\frac{\partial E(x,y)}{\partial w_k} = d_k q_k(w_f F_{y,k}^{f} g_{\sigma_f}(x, x_k + w_k) + w_b F_{y,k}^{b} g_{\sigma_b}(x, x_k + w_k)),
\label{eq:grad_wk}
\end{equation}
\begin{equation}
\frac{\partial E(x,y)}{\partial d_k} = q_k(w_f F_{x,k}^{f} F_{y,k}^{f} + w_b F_{x,k}^{b} F_{y,k}^{b}).
\label{eq:grad_dk}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=0.55\linewidth]{DAC26-OMPC-sub/figs/shot_202511.pdf}
    \caption{Variation in execution time of exact and fast method with respect to the number of shots.}
    \label{fig:shot_202511}

\end{figure}

In order to enhance computational efficiency while maintaining differentiability, we construct a fast version of the energy deposition computation. The energy deposition can be expressed as the convolution of the PSF with the dose $M_d(x,y)$:
\begin{equation}
E_{\text{fast}}(x,y) = P(r) \otimes M_d(x,y), \quad r = \sqrt{x^2 + y^2}.
\label{fig:E_fast}
\end{equation}

To construct $M_d(x,y)$, we employ smoothed rectangular window functions based on the erf, expressed as:
\begin{equation}
M_d(x,y) = \sum_{k=1}^N d_k \, E_{k, \sigma'}(x,y),
\label{eq:md}
\end{equation}
where $E_{k, \sigma'}(x,y)$ is similar in form to that in \Cref{eq:Ek_sigma} but differs in that it transforms the discrete shot dose distribution into a differentiable pixel-level dose map, enabling gradient-based optimization. The hyperparameter $\sigma'$ controls the edge steepness of the window.

The fast Fourier transform (FFT) can be employed to accelerate this computation. We further benchmarked the runtime of both fast and exact methods across varying shot counts. As shown in \Cref{fig:shot_202511}, as the number of shots increases, the fast method increasingly outperforms the exact one. Meanwhile, \Cref{fig:model_error_new} shows that this acceleration incurs only a very slight loss in accuracy, which remains below $10^{-3}$.

\subsection{MDP via Shot-Level Optimization}
Given an ideal curvilinear mask generated by ILT, we first fracture it into rectangular shots using the method in~\cite{fracture}, obtaining a coarse initial solution. We then perform shot-level MDP optimization using the proposed differentiable EBL simulator. The framework jointly optimizes mask fidelity and manufacturability through the following composite loss function:
\begin{equation}
L = \alpha_1 L_2  + \gamma_1 L_s + \delta_1 L_{\text{d}} + \epsilon_1 L_{\text{o}},
\label{eq:loss}
\end{equation}
where the sparsity regularizer $L_s$, which reflects the number of activated shots, encourages shot efficiency and is defined as:
\begin{equation}
L_s = \sum_{k=1}^N q_k.
\label{eq:sparsity}
\end{equation}

The total dose loss $L_{\text{d}}$ reflects the cumulative dose of VSB shots:
\begin{equation}
L_{\text{d}} = \sum_{k=1}^N w_k \cdot h_k \cdot d_k \cdot q_k.
\label{eq:dose}
\end{equation}

The overlap loss $L_{\text{o}}$ penalizes redundant coverage between shots:
\begin{equation}
L_{\text{o}} = \sum_{k=1}^N \sum_{p=k+1}^N A_{\text{overlap}}(k,p) \cdot q_k \cdot q_p.
\label{eq:overlap}
\end{equation}

The $L_2$ term measures the Euclidean distance between the target and simulated mask. Its gradient with respect to $x_k$ is given in \Cref{eq:mpc_loss_g}, while gradients with respect to $y_k$, $w_k$, $h_k$, $d_k$, and $q_k$ are derived similarly.

\begin{equation}
\frac{\partial L_2}{\partial x_k} = \sum_{x,y} \frac{\partial L_2}{\partial Z_e(x,y)} \frac{\partial Z_e(x,y)}{\partial E(x,y)} \frac{\partial E(x,y)}{\partial x_k}.
\label{eq:mpc_loss_g}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{DAC26-OMPC-sub/figs/model_error_new.pdf}
    \caption{(a) Energy deposition distribution obtained via the fast method. (b) Energy deposition distribution obtained via the exact method. (c) Absolute error of the fast method relative to the exact method.}
    \label{fig:model_error_new}
\end{figure}
As presented by \Cref{alg:mdp_opt}, our shot-level MDP optimization method consists of the following steps:

Initialization: We start with an initial shot set $\mathbb{S}$. All shots are first projected into their feasible ranges using the STE or clipping functions (lines 5-9), ensuring that all constraints on position, size, dose, and active flag are satisfied.

Forward EBL Simulation: At each optimization step, the current shot set $\tilde{\mathbb{S}}$ is fed into a differentiable EBL simulator to predict the resulting mask pattern $M_t$ (line 11).

Loss Computation: At each optimization step, the loss $L$ is computed based on the current shot set $\tilde{\mathbb{S}}$, mask pattern $M_t$, and the target mask $\mathbf{T}$ (line 13).

Gradient-Based Update: Gradients of the loss with respect to the shot parameters are computed via backpropagation (line 15), and the shot set is updated using gradient descent (line 16) to reduce the loss. The learning rate is halved at the midpoint of optimization to improve convergence stability. The best-performing shot set $\mathbb{S}^*$ is saved whenever the loss improves.

\begin{algorithm}[tb!]
\caption{\textbf{Shot-Level MDP Optimization}}
\label{alg:mdp_opt}
\begin{algorithmic}[1]
\State \textbf{Input:} Initial shot set $\mathbb{S} = \{(x_k, y_k, w_k, h_k, d_k, q_k)\mid k = 1, 2, \dots, N \}$, 
target mask $\mathbf{T}$, EBL parameters $(\sigma_f, \sigma_b, \eta, \theta_z, E_\mathit{th})$, 
shot constraints $[w_\text{min}, w_\text{max}, h_\text{min}, h_\text{max}, d_\text{min}, d_\text{max}]$, 
learning rate $l_r$, epochs $\mathbb{N}$.
\State \textbf{Output:} Optimized shot set $\mathbb{S}^*$
\vspace{2pt}

\For{$t = 1$ to $\mathbb{N}$}
    \State \textbf{// 1. Constraint enforcement}
    \State $\tilde{x}_k, \tilde{y}_k \gets \text{STE}((x_k, y_k), [0, M-1])$
    \State $\tilde{w}_k, \tilde{h}_k \gets \text{STE}((w_k, h_k), [w_\text{min}, w_\text{max}], [h_\text{min}, h_\text{max}])$
    \State $\tilde{d}_k \gets \text{clip}(d_k, d_\text{min}, d_\text{max})$
    \State $\tilde{q}_k \gets \text{STE}(\text{clip}(q_k, 0, 1))$
    \State $\tilde{\mathbb{S}} \gets \{\tilde{x}_k, \tilde{y}_k, \tilde{w}_k, \tilde{h}_k, \tilde{d}_k, \tilde{q}_k\}$

    \State \textbf{// 2. Forward EBL simulation}
    \State $M_t \gets \text{EBL}(\tilde{\mathbb{S}})$

    \State \textbf{// 3. Compute total loss}
    \State $L \gets \text{Loss}(\tilde{\mathbb{S}}, M_t,\mathbf{T})$

    \State \textbf{// 4. Gradient update}
    \State $\nabla_{\tilde{\mathbb{S}}} L \gets \text{backprop}(L)$
    \State $\mathbb{S} \gets \tilde{\mathbb{S}} - l_r \nabla_{\tilde{\mathbb{S}}} L$
    
    \If{$t = \mathbb{N}/2$} $l_r \gets l_r / 2$ \EndIf
    \State Save $\mathbb{S}^*$ if $L$ improved
\EndFor

\State \Return $\mathbb{S}^*$
\end{algorithmic}
\end{algorithm}



\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{DAC26-OMPC-sub/figs/MDP-ILT_202511.pdf}
    \caption{Overall Flow of our unified framework.}
    \label{fig:MDP_ILT_202511}

\end{figure*}

\subsection{MDP-based ILT}
The objective of the MDP stage is to generate a real mask that closely matches the given ideal mask. However, the ultimate goal of mask optimization is to achieve high wafer pattern fidelity rather than mask pattern fidelity. To this end, we extend pixel-level mask optimization into an MDP-based ILT. Since both the EBL and OL simulations are fully differentiable, our unified framework enables gradient-based optimization of shot parameters, as illustrated in \Cref{fig:MDP_ILT_202511}. The industry standard employs a $4:1$ reduction system, in which mask patterns are $4\times$ larger than the corresponding wafer patterns. Accordingly, during the MDP stage, the wafer-level pattern is magnified by 4× to produce the mask-level pattern, and subsequently reduced by 4× in the OL stage to restore wafer-scale dimensions, ensuring compatibility with the OL simulator. Notably, we first apply curvilinear design retargeting (CDR) to the original layout before optimization. This preprocessing step is motivated by the observation that both OL and EBL act as low-pass filters, attenuating high-frequency features such as sharp corners that cannot be faithfully transferred onto the wafer. Directly optimizing these high-frequency regions may cause overfitting and degrade overall performance. Following the approach in~\cite{cdr}, we therefore adopt the CDR-processed layout as the optimization target. Nevertheless, all evaluations are performed with respect to the original target layout to ensure a fair assessment of pattern fidelity. The multi-objective loss function for this optimization is defined as:
\begin{equation}
L = \alpha_2 L_2 + \beta_2 L_{\text{pvb}} + \gamma_2 L_s + \delta_2 L_{\text{d}} + \epsilon_2 L_{\text{o}},
\label{eq:loss}
\end{equation}
where $L_2$ represents the Euclidean distance between the final wafer pattern and the target layout. Compared with the loss function used in the MDP stage, the PVB term is additionally incorporated to improve process robustness.
The gradient flow from the squared $L_2$ loss to $x_k$ can be formulated as:
\begin{equation}
\frac{\partial L_2}{\partial x_k} = \sum_{x,y} \frac{\partial L_2}{\partial Z_p(x,y)} \frac{\partial Z_p(x,y)}{\partial Z_e(x,y)} \frac{\partial Z_e(x,y)}{\partial E(x,y)} \frac{\partial E(x,y)}{\partial x_k}.
\label{eq:ompc_loss_g}
\end{equation}
The gradients of the squared $L_2$ and PVB losses with respect to the remaining shot parameters can be derived analogously.
